Privacy Amplification via Shuffled Check-Ins

We study a protocol for distributed computation called shuffled check-in, which achieves strong privacy guarantees without requiring any further trust assumptions beyond a trusted shuffler. Unlike most existing work, shuffled check-in allows clients to make independent and random decisions to participate in the computation, removing the need for server-initiated subsampling. Leveraging differential privacy, we show that shuffled check-in achieves tight privacy guarantees through privacy amplification, with a novel analysis based on R{\'e}nyi differential privacy that improves privacy accounting over existing work. We also introduce a numerical approach to track the privacy of generic shuffling mechanisms, including Gaussian mechanism, which is the first evaluation of a generic mechanism under the distributed setting within the local/shuffle model in the literature. Empirical studies are also given to demonstrate the efficacy of the proposed approach.

==> app_additional.tex <==
\section{Code for Reproducibility}
\label{app:code}
See \url{https://anonymous.4open.science/r/checkin-B2B1/} for the code of our implementation.

\section{Additional Privacy Analyses}
\label{app:add}
\subsection{Distributed check-in under removal DP}
\label{subsec:rm_dci}
As before, we assume that the server aggregates the received messages by outputting the average, $\frac{1}{B}\sum_{i=1}^B x_i + \mathcal{N}(0,\sigma^2/B)$.
The mechanism is closely related to Poisson subsampling \citep{zhu2019poission}.

\begin{theorem}
[Distributed check-in Gaussian RDP (removal DP)]
Consider the mechanism in Equation \ref{eq:cci} where agg is a mean operation on collected values.
Here it is assumed that the adversary does not know the number of user checking in in each round.
\begin{align}
\eps(\lambda) &\leq \frac{1}{1-\lambda}\log \{(1-\gamma)^{\lambda-1}(\lambda\gamma-\gamma+1) \nonumber \\
&+ \sum_{k=1}^{n-1}\binom{\lambda}{2}\binom{n-1}{k}\gamma^{k+2} (1-\gamma)^{n+\lambda-3-k} e^{\eps_k^{\rm CCI}(2)} \label{eq:poiss1} \\
&+ \binom{\lambda}{2}(1-\gamma)^{n+\lambda-3}\gamma^2 e^{1/\sigma^2} + 3 \sum_{l=3}^\lambda\binom{\lambda}{l} \gamma^{\lambda-l} (1-\gamma)^{n+l-1}e^{l(l-1)/2\sigma^2} \nonumber \\
&+ 3\sum_{k=1}^{n-1}\sum_{l=3}^\lambda \binom{n-1}{k} \binom{\lambda}{l}\gamma^{k+\lambda-l} (1-\gamma)^{n+l-1-k}e^{(l-1)\eps_k^{\rm CCI}(l)}\} \label{eq:poiss2}
\end{align}
where $\exp((l-1)(\eps_k^{\rm CCI}(l)) = \sqrt{\frac{(k+1)^{l}}{(k+l)k^{l-1}}}\exp{(-\frac{l+1}{\sigma^2(k+1)})}$ for $k\geq 1 $.
% and $\eps_0^{\rm CCI}(l) = l/2\sigma^2$.
Line \ref{eq:poiss1} can be further approximated as
\begin{align}
   \binom{\lambda}{2}\gamma^2 (1-\gamma)^{\lambda-2} \left(e^{\eps_{1}^{\rm CCI}(2)-\Delta^2(n-1)\gamma/2} + e^{\eps_{(1-\Delta)(n-1)\gamma+1}^{\rm CCI}(2)}\right)
\end{align}
and Line \ref{eq:poiss2} can be further approximated as
\begin{align}
% \eps(\lambda) &\leq \frac{1}{1-\lambda}\log \{(1-\gamma)^{\lambda-1}(\lambda\gamma-\gamma+1) \nonumber \\
% &+ \binom{\lambda}{2}\gamma^2 (1-\gamma)^{\lambda-2} e^{\eps^{\rm CCI}(2)} + 3 \sum_{l=2}^\lambda (1-\gamma)^{n-1}(1-\lambda)^{l}\lambda^{\lambda-l}e^{l(l-1)/2\sigma^2} \nonumber \\
3\sum_{l=2}^\lambda  \binom{\lambda}{l}(1-\gamma)^{l}\gamma^{\lambda-l}(e^{(l-1)\eps_{1}^{\rm CCI}(l)-\Delta^2(n-1)\gamma/2}+e^{(l-1)\eps_{(1-\Delta)(n-1)\gamma+1}^{\rm CCI}(l)})
\end{align}
where $\Delta \in [0,1]$.
\end{theorem}
\begin{proof}
The neighboring databases are $D$, $D' = D \cup \{x\}$, and the mechanisms acting on them are $\mathcal{M},\mathcal{M'}$ respectively.
Let $J$ be the index set indicating whether a user participates in training, $J=  (\sigma_1,\sigma_2,\cdots,\sigma_n) \in \{0,1\}^n$.
Let $\mathbb{P}(J)$ be the probability distribution of $J$.

We denote $q(J)$ by the underlying randomization mechanism, which is a Gaussian mechanism with variance $\sigma^2/k$, $k$ being the number of non-zero elements in $J$.
Following \cite{zhu2019poission}, we define $q' = \sum_J q'(J), q'(J) = q(\sigma_1, \cdots, \sigma_{n-1}, 1)$, and similarly $p(J)=p'(J) = q(\sigma_1, \cdots, \sigma_{n-1}, 0)$.
We have $q = (1-\gamma)p + \gamma q'$ or $p = q+\gamma p'-\gamma q'$.

we want to calculate the RDP of neighboring databases $\mathcal{M}\sim p$, $\mathcal{M'}\sim q$:
\begin{align*}
&\mathbb{E}_{\mathcal{M'}}\left[(\mathcal{M}/\mathcal{M'})^\lambda\right] = \mathbb{E}_q \left[\left(\frac{q+\gamma p'-\gamma q'}{q}\right)^{\lambda}\right] \\
& \leq \mathbb{E}_{\sigma_1,\dotsc,\sigma_{n-1}} \{\gamma \mathbb{E}_{q'(J)}\left(\frac{(1-\gamma)q'(J)+\gamma p'(J)}{q'(J)}\right)^{\lambda}  + (1-\gamma) \mathbb{E}_{p'(J)}\left(\frac{(1+\gamma)p'(J)-\gamma q'(J)}{p'(J)}\right)^{\lambda} \} \\
& = \sum_{k=0}^{n-1}\sum_{l=0}^{\lambda} \binom{\lambda}{l} \binom{n-1}{k}\gamma^k (\gamma)^{n-1-k}  (1-\gamma)^{\lambda-l}\gamma^l \left\{\gamma\mathbb{E}_{q'(k)} \left(\frac{{p'(k)}}{{q'(k)}}\right)^{l} + (1-\gamma)\mathbb{E}_{p'(k)}\left(2-\frac{{q'(k)}}{{p'(k)}}\right)^{l}\right\}
\end{align*}
Here, $q'(k)\sim \mathcal{N}(1/(k+1),\sigma^2/(k+1))$, $p'(k)\sim \mathcal{N}(0,\sigma^2/k)$ when $k\geq 1$.
By direct computation $\mathbb{E}_{q'(k)}(p'(k)/q'(k))^{\lambda} = \sqrt{\frac{(k+1)^{\lambda}}{(k+\lambda)k^{\lambda-1}}}\exp{(-\frac{\lambda+1}{\sigma^2(k+1)})}$. 
When $k=0$, $q'(k)\sim \mathcal{N}(1,\sigma^2)$, $p'(k)\sim \mathcal{N}(0,\sigma^2)$ and $\mathbb{E}_{q'(k)}(p'(k)/q'(k))^{\lambda} = \exp{[(\lambda^2-\lambda)/(2\sigma^2)]}$.

Moreover, from Lemma \ref{lm:chernoff}, we can make the approximation of lines \ref{eq:poiss1} and \ref{eq:poiss2}.
% From the Chernoff bound:  $\mathbb{P}[X \leq (1-\Delta)\mu] \leq e^{-\Delta^2\mu/2}$ for all $\Delta \in [0,1]$ and the union of probability, we can make the approximation of lines \ref{eq:poiss1} and \ref{eq:poiss2}.

We can then use the same argument in \cite{zhu2019poission} to obtain the desired result.

% We can write $\tilde{q}(k) = \sum_{J}\mathbb{P}(J)q(J)\delta(\sum_i\sigma_i=k)=\binom{n}{k}\gamma^k(1-\gamma)^{n-k}\mathcal{N}(1/k,\sigma^2/k)$.
\end{proof}
\begin{remark}
One can obtain a tighter bound if $\mathbb{E}_{q'(k)}(p'(k)/q'(k)-1)^{\lambda}\geq 0$ for odd $\lambda$ \citep{zhu2019poission}.
Unfortunately this does not apply to our scenario as $\mathbb{E}_{q'(k)}(p'(k)/q'(k)-1) <0$ by direct computation.
\end{remark}

% \subsection{Shuffled check-in with discrete $\eps_0$-LDP randomizer}
% \label{subsec:upplow}
% A variety of discrete $\eps_0$-LDP SGD methods has been applied to distributed learning \cite{bhowmick2018protection,erlingsson2020encode,girgis2021shuffled}.
% Roughly speaking, the following procedures are taken in these algorithms: clients clip the $l_p$-norm ($p\in [1,\infty]$) of the gradient, apply an $\eps_0$-LDP mechanism to randomize and represent the clipped gradient with a finite number of bits, and send it to the server.
% We provide the RDP bounds on these types of mechanism, beginning with the upper bound.
% \begin{theorem}[Upper Bound]
% \label{th:upper}
% For any $\eps_0\geq 0$, $n\in \mathbb{N}$, $l\leq n$ such that $n\gamma = l$ ($0\leq\gamma \leq 1$), and any integer $\lambda\geq 2$, the RDP of the shuffled check-in mechanism (Equation \ref{th:main}) is upper-bounded by $\eps(\lambda)\leq\frac{1}{\lambda-1}\log\left(\mathbb{E}\left[\left(\frac{\calM(D)}{\calM(D')}\right)^{\lambda}\right]\right)$, where
% \begin{align}
% \label{eq:upper}
%     \mathbb{E}\left[\left(\frac{\calM(\calD)}{\calM(\calD')}\right)^{\lambda}\right]
% &\leq 1 + 4\binom{\lambda}{2}\gamma^{2}\left(e^{\epsilon_0}-1\right)^2 \left( e^{-\epsilon_0-\Delta^2n\gamma/2} + e^{-\epsilon_0}/\Tilde{l} \right) \nonumber \\
% &+ \sum_{j=3}^{\lambda}\binom{\lambda}{j}\gamma^{j} j \Gamma\left(j/2\right) \left(\frac{2\left(e^{2\epsilon_0}-1\right)^2}{e^{2\epsilon_0}}\right)^{j/2}\left(e^{-\Delta^2 n\gamma/2} + \Tilde{l}^{-j/2} \right) \nonumber \\
% &+\Upsilon_1 e^{-\Delta^2 n\gamma/2} + \Upsilon_{(1-\Delta)n\gamma+1}.
% \end{align}
% Here, $0 \leq \Delta \leq 1$ is arbitrary, $\Tilde{l}=\floor{\frac{(1-\Delta)n\gamma}{2\eps_0}}+1$, $\Gamma\left(z\right)=\int_{0}^{\infty}x^{z-1}e^{-x}dx$ is the Gamma function, $\Upsilon_k$ is given by $\Upsilon_k=\left(\left(1+\gamma \frac{e^{2\epsilon_0}-1}{e^{\epsilon_0}}\right)^{\lambda}-1-\lambda\gamma \frac{e^{2\epsilon_0}-1}{e^{\epsilon_0}}\right)e^{-\frac{k-1}{8e^{\epsilon_0}}}$.
% \end{theorem}
% % \noindent \textit{Proof sketch.}
% \begin{proof}[Proof sketch.]
% Here, we give an outline of the proof.
% We notice from Equation \ref{eq:main} that inside the logarithm is a summation over $k$ of the expected moments of a subsampled without replacement (with $k$ data instances), shuffle mechanism.
% We first obtain a bound on the latter using the results from \cite{girgis2021renyib}.
% Then, the summation over $k$ is bounded using the properties of the expected moments and the Chernoff bound.
% The full proof is available in Appendix \ref{app:proof}.
% \end{proof}

% While Equation \ref{eq:upper} may seem complicated, it is necessary as we attempt to obtain a precise expression (instead of an order approximation).
% This is particularly critical when considering deployment in real-life private systems, as constants matter \cite{wang2019subsampled}.
% Some numerical issues related to its evaluation will be discussed in later remarks and sections.

% We next provide the corresponding lower bound.
% \begin{theorem}[Lower Bound]
% \label{th:lower}
% For any $\eps_0\geq 0$, $n\in \mathbb{N}$, $l\leq n$ such that $0\leq\gamma \leq 1$, and any integer $\lambda\geq 2$, the RDP of the shuffled check-in mechanism (Equation \ref{th:main}) is lower-bounded by
% \begin{equation}
% \label{eq:lower}
%     \eps(\lambda)\geq\frac{1}{\lambda-1}\log\left(
% 1+ (1-e^{-\Delta^2n\gamma/(2+\Delta)})\binom{\lambda}{2}\gamma^2\frac{\left(e^{\epsilon_0}-1\right)^2}{(1+\Delta)n\gamma e^{\epsilon_0}}
% \right),
% \end{equation}
% where $0 \leq \Delta \leq 1$ is arbitrary.
% \end{theorem}
% % \noindent \textit{Proof sketch.}
% \begin{proof}[Proof sketch.]
% The lower bound is calculated assuming that the underlying $\eps_0$-LDP discrete mechanism is a binary randomized response.
% Again, we first obtain the expression of the subsampled without replacement (with $k$ data instances), shuffle binary randomized response.
% Using the properties of the expression as well as the Chernoff bound, we place a lower bound on the RDP.
% For the full proof, see Appendix \ref{app:proof}.
% \end{proof}
% \noindent \textit{Proof sketches.}
% We give an outline of the proof of Theorem \ref{th:upper} and \ref{th:lower}. \footnote{The full proof can be found in Appendix \ref{app:proof}.}
% As can be seen from Theorem \ref{th:main}, 

% Several remarks on the bounds are in line.
% \begin{remark}
% The value $\Delta$ comes from the Chernoff bound.
% While we can optimize this value to provide tighter bounds, we typically use $\Delta = 1/2$ as it gives reasonably good results, and simplifies the evaluation.
% \end{remark}

% \begin{remark}
% \label{rm:logl}
% Converting the RDP bounds to approximate DP requires the use of Lemma \ref{lm:rdpdp}, which is a quasi-convex optimization problem given $\eps(\lambda)$, solvable in logarithmic time.
% As the computational cost of Equation \ref{eq:upper} is $O(\lambda)$ (assuming that we fix a maximum $\lambda$), the overall computational cost is $O(\lambda\log(\lambda))$.
% \end{remark}

% \begin{remark}
% One may further close the gap between the upper and lower bounds under the following conditions.
% A tighter upper bound may be obtained by considering specific subsampled shuffle mechanism.
% Meanwhile, a tighter lower bound may be obtained by carefully bounding the binomial distribution central moments (see Appendix \ref{app:proof}), at the sacrifice of the expression's (Equation \ref{eq:lower}) simplicity.
% \end{remark}

\subsection{Shuffled check-in with a generic $(\eps_0,\delta_0)$-LDP randomizer}
Here, we give another approach of privacy accounting of shuffled check-in with a generic $(\eps_0,\delta_0)$-LDP randomizer, following arguments given at the end of Section \ref{subsec:rdp_sci}.

\noindent\textbf{Shuffling conversion.}
\begin{enumerate}
    \item Convert shuffle DP to shuffle RDP.
    \item Use shuffle RDP to evaluate subsampled shuffle RDP
    \item Substitute it into Equation \ref{eq:main} to evaluate the composition of RDP.
\end{enumerate}
To calculate the shuffle DP with $(\eps_0,\delta_0)$-LDP randomizer, we use Theorem 3.8 given by \cite{feldman2022hiding}. 
% \footnote{\label{fn:shuff}.
% The result of privacy amplification by shuffling by \cite{feldman2022hiding} is valid only when $\eps_0 \leq \log\left(n/16\log(2/\delta)\right)$. For parameters violating this condition, we assume that no amplification occurs, i.e., $\eps=\eps_0$. 
% This is well corroborated by the numerical experiments performed in \cite{feldman2022hiding}.}
The subsampled RDP can be calculated using Theorem 9 of \cite{wang2019subsampled}.

Note that Step 2 is a calculation of $O(\lambda)$ in terms of time complexity \citep{wang2019subsampled}.
Step 3 involves evaluating the summation with respect to $n$ as in Equation \ref{eq:main}, which is of $O(n)$.
One also needs to convert the RDP notion back to approximate DP using Lemma \ref{lm:rdpdp}, which is an $O(\lambda)$ operation.
% Overall, the shuffling conversion approach is of time complexity $O(n\lambda^2)$. \footnote{Here, we do not include the time complexity of optimizing Equation \ref{eq:dprdp} for convenience as it is irrelevant to the subsequent discussions.
% We note however that Equation \ref{eq:dprdp} is convex optimization problem which can be solved efficiently.}

% Table \ref{tab:comp} summarizes the 
Table \ref{tab:comp} summarizes the two approaches introduced in this paper.
Although the subsampling shuffling conversion approach has lower time complexity, we expect the RDP bound to be looser than the shuffling conversion approach as the conversion to RDP occurs one step later.

\begin{table}
\begin{center}
\caption{Our approaches to bounding shuffled check-in mechanism with a generic $(\eps_0,\delta_0)$-LDP randomizer.
Here, A, B, C, D refer to techniques used in \cite{feldman2022hiding}, \cite{wang2019subsampled}, \cite{balle2018privacy},  \cite{balle2018privacy}, respectively.
See text for details.
    The conversion from DP to RDP (using Lemma \ref{lm:dprdp}) can be performed in two different steps leading to different time complexities as shown in the Table.
    Dependence of the time complexity on other factors is suppressed.}
    \label{tab:comp}

    \begin{tabular}{ccccc}
        \toprule
        %\multirow{2}{*}{Dataset} &  \multicolumn{3}{c|}{social}& comm & web \\
        
         &Shuffling&  Subsampling& Convert to RDP from & Time complexity \\
                \midrule
      Shuff. conv.& Use A (DP) &Use B (RDP)& A& $O(n\lambda^2)$ \\
      Subs. shuff. conv.& Use A (DP)& Use C (DP)& A+D& $O(n \lambda)$ \\
    %   Processing complexity& -& $n^2$& $O(\log(n))$ \\
        \bottomrule
    \end{tabular}
    
\end{center}
% \vspace{-0.2cm}
\end{table}


==> intermediate.tex <==
\section{Self Check-in}
\subsection{Model-independent protocol and expression}
Let us begin by describing the protocol of self check-in.
In each round $t$, a message is broadcast to all clients to ask for participation in the learning.
Each client flips a biased coin to decide whether to participate in the training.
The probability of a client participating in the training successfully is modeled by a parameter $\gamma$ ($0 \leq \gamma \leq 1$), which we call the \textit{check-in rate}.
The participating probability follows the Bernoulli distribution, Bern($\gamma$).
In Section \ref{subsec:prac}, we discuss how to determine $\gamma$ in practice.

Clients decided to participate download the model $\theta_t$, calculate the gradient, apply local randomizer to it (e.g., clip the gradient norm and add Gaussian noise), and send it (encrypted) to a shuffler or aggregator, depending on the trust model.
% The shuffler permutes randomly all the received messages before forwarding them to the untrusted aggregator if the shuffler is used.
% Otherwise, 
Then, the aggregator updates the model parameters to $\theta_{t+1}$ using the messages processed by the shuffler or SecAgg.
The underlying (trust) model-dependent mechanism is denoted by \textit{base mechanism}.
Next, we give the model-independent expression of the RDP of self check-in.

\begin{theorem}[RDP of self check-in]
\label{th:main}
Let $D,D'$ be adjacent databases consisting of $n$ clients, and $\gamma$ the (effective) check-in rate.
The RDP of order $\lambda$ of the self check-in mechanism is bounded by
\begin{equation}
    \eps(\lambda) \leq \frac{1}{\lambda-1} \log \left(
    \sum_{k=0}^{n}  \binom{n}{k} \gamma^{k} (1-\gamma)^{n-k} \mathbb{E}_{q_k^{\rm s}}\left[\left(\frac{p_k^{\rm s}}{q_k^{\rm s}}\right)^{\lambda}\right]
    \right).
    \label{eq:main}
\end{equation}
Here, $p_k^{\rm s}$ is the output probability distribution of the subsampled without replacement (of $k$ data instances) base mechanism.
$q_k^{\rm s}$ is the output probability distribution induced by the same mechanism but on $D'$. 
\end{theorem}
\begin{proof}
% We first note that the self check-in mechanism $\calM$ can be seen to be a mechanism outputting a subset of data of range $S$.
% We first note that the self check-in mechanism $\calM$ can be written as $\calM : \calD^n \to 2^n \times \calS^n$, as it outputs a subset (indicated by the range, $2^n$) of data of range $S$.
Let us first give the following observation.
Under the shuffle model, $k$ data instances perturbed by a LDP randomizer $\calA:\calD \to \calS$ check in to undergo shuffling for $k \in [n]$;
under distributed DP, $k$ data instances check in to be processed by, e.g., SecAgg, to return a perturbed aggregated output without exposing individual information, $\text{agg}:\calD^k \to \calS$ for $k \in [n]$.
Notice that there are two output variables for the self check-in mechanism $\calM$: $k \in [n]$, the number of data instances, and $\phi \in \calS$, the randomized content of each data instance (shuffler) or the aggregated output (distributed DP).

As clients check in independently with a probability of $\gamma$, the total number of clients checking in distributes as a binomial distribution.
Hence, following the observation given above on the output variables, the neighboring mechanism may be written as 
\begin{align*}
\calM(\calD)(k,\phi)\sim   \binom{n}{k} \gamma^{k} (1-\gamma)^{n-k} p_k^{\rm s}, \; \; 
\calM(\calD')(k,\phi)\sim \binom{n}{k} \gamma^{k} (1-\gamma)^{n-k} q_k^{\rm s}. 
\end{align*}

This gives the expression of Equation \ref{eq:main} following the definition of RDP.
To complete the proof, we need to show that $p_k^{\rm s}$ is the probability distribution of a subsampled (without replacement) mechanism.
For brevity, we write $p_k^{\rm s}$ and $q_k^{\rm s}$ as $p_k$ and $q_k$ respectively.
We note that both $p_k$ and $q_k$ are mixture distributions consisting of distribution with (and without) the differing data instance.
More precisely, let the differing data instance be the $n$-th item of $D,D'$.
Let $E$ be the subset containing the $n$-th item ($E^c$ the subset with the complementary item).
Subsequently,
$$
p_k = (1-\gamma)p_k(\cdot|E^c) + \gamma p_k(\cdot|E), \quad q_k = (1-\gamma)q_k(\cdot|E^c) + \gamma q_k(\cdot|E)
$$
and $p_k(\cdot|E^c) = q_k(\cdot|E^c)$.
This expression is by definition the distribution corresponding to the subsampling without replacement scenario \citep{wang2019subsampled}.
Plugging the above expressions to Equation \ref{eq:rdpdiv}, we obtain Equation \ref{eq:main} as desired.
\end{proof}
% This allows us to leverage known behaviors of subsampling and shuffling to calculate the RDP of shuffled check-in, as described in the next section.
\begin{remark}
Theorem \ref{th:main} states that the self check-in's RDP is effectively composed of the RDP of a subsampled version of the base mechanism weighted by a binomial distribution.
As stated before, one can simply plug the model-dependent base mechanism into this model-independent expression to calculate the specific RDP, as will be demonstrated in the next section.
% As stated before, this is an expression applicable to any base mechanism which may be self check-in distributed protocol (where each client decides to participate in the training with a certain probability) irrespective of the base mechanism, which can be plugged in to the expression, as will be demonstrated in the next section.
\end{remark}
\begin{remark}
It is recently shown that performing even tighter privacy accounting is possible via privacy loss distributions (which may be seen as a scaled RDP divergence of order 1) and fast Fourier transforms \citep{koskela2020computing,gopi2021numerical}.
These techniques are however limited to distributions that can be reduced to a one-dimensional problem, and therefore not applicable to self check-in as in Equation \ref{eq:main}, a high-dimensional mixture distribution of $n$ components.
See Section 5 of \cite{koskela2021tight}, where a similar problem occurs in the shuffle model.
It is henceforth more appropriate to attack the privacy composition problem of self check-in with RDP.
\end{remark}

\subsection{Practical considerations}
\label{subsec:prac}
In our protocol, each client carries a $p$-biased coin such that she would decide to participate in the training only when head is returned.
Even after a client decides to participate, she may \textit{drop out} due to various reasons as discussed in Introduction.
Assuming that clients have a certain constant and independent probability of dropping out, $p'$, the \textit{effective} check-in rate is then $\gamma = p(1-p')$.
A practitioner can choose to determine the empirical $\gamma$ (by monitoring the number of client checking in in each round), or conservatively use $p$ as the check-in rate to yield a valid privacy upper bound (as smaller check-in rate leads to larger amplification).
These henceforth allow for robust modelling of dropouts.
% Hence, a practitioner should monitor the number of client checking in in each round and determine the empirical $\gamma$ instead of simply using $p$ as the check-in rate to model dropouts robustly. 
Moreover, instead of treating $p'$ as a constant, one could further better model the dropout rate as, e.g., a time-dependent function, as in reliability engineering \citep{bazovsky2004reliability}, but we leave this system-dependent and slightly orthogonal consideration for future work.

\section{Self Check-in with intermediate trust models}
Using Theorem \ref{th:main}, we next show how to integrate self check-in with intermediate trust models as a realization of private FL.

\subsection{RDP for shuffled check-in}
\label{subsec:rdp_sci}
Let shuff be the shuffling mechanism that randomly permutes any number of received messages and outputs them. The shuffled check-in mechanism can then be written formally as
\begin{equation}
    \calM(D) := \text{shuff}(\{\calA(x_i)| \sigma_i=1, i \in [n]\}), \quad \sigma_i \sim \text{Bern}(\gamma).
\end{equation}

\textbf{Discrete $\eps_0$-LDP randomizer.}
We first consider shuffling of discrete-value $x_i$ perturbed by an $\eps_0$-LDP randomizer, of which has been applied to distributed learning \citep{bhowmick2018protection,erlingsson2020encode,girgis2021shuffled}.
Roughly speaking, the following procedures are taken in these algorithms: clients clip the $l_p$-norm ($p\in [1,\infty]$) of the gradient, apply an $\eps_0$-LDP mechanism to randomize and represent the clipped gradient with a finite number of bits, and send it to the server.
We provide the RDP bounds on these types of mechanism, beginning with the upper bound.
\begin{theorem}[Upper Bound]
\label{th:upper}
For any $\eps_0\geq 0$, $n\in \mathbb{N}$, $l\leq n$ such that $n\gamma = l$ ($0\leq\gamma \leq 1$), and any integer $\lambda\geq 2$, the RDP of the shuffled check-in mechanism is upper-bounded by $\eps(\lambda)\leq\frac{1}{\lambda-1}\log\left(\mathbb{E}\left[\left(\frac{\calM(D)}{\calM(D')}\right)^{\lambda}\right]\right)$, where
\begin{align}
\label{eq:upper}
    \mathbb{E}\left[\left(\frac{\calM(\calD)}{\calM(\calD')}\right)^{\lambda}\right]
&\leq 1 + 4\binom{\lambda}{2}\gamma^{2}\left(e^{\epsilon_0}-1\right)^2 \left( e^{-\epsilon_0-\Delta^2n\gamma/2} + e^{-\epsilon_0}/\Tilde{l} \right) \nonumber \\
&+ \sum_{j=3}^{\lambda}\binom{\lambda}{j}\gamma^{j} j \Gamma\left(j/2\right) \left(\frac{2\left(e^{2\epsilon_0}-1\right)^2}{e^{2\epsilon_0}}\right)^{j/2}\left(e^{-\Delta^2 n\gamma/2} + \Tilde{l}^{-j/2} \right) \nonumber \\
&+\Upsilon_1 e^{-\Delta^2 n\gamma/2} + \Upsilon_{(1-\Delta)n\gamma+1}.
\end{align}
Here, $0 \leq \Delta \leq 1$ is arbitrary, $\Tilde{l}=\floor{\frac{(1-\Delta)n\gamma}{2\eps_0}}+1$, $\Gamma\left(z\right)=\int_{0}^{\infty}x^{z-1}e^{-x}dx$ is the Gamma function, $\Upsilon_k$ is given by $\Upsilon_k=\left(\left(1+\gamma \frac{e^{2\epsilon_0}-1}{e^{\epsilon_0}}\right)^{\lambda}-1-\lambda\gamma \frac{e^{2\epsilon_0}-1}{e^{\epsilon_0}}\right)e^{-\frac{k-1}{8e^{\epsilon_0}}}$.
\end{theorem}
% \noindent \textit{Proof sketch.}
\begin{proof}[Proof sketch.]
Here, we give an outline of the proof.
We notice from Equation \ref{eq:main} that inside the logarithm is a summation over $k$ of the expected moments of a subsampled without replacement (with $k$ data instances), shuffle mechanism.
We first obtain a bound on the latter using the results from \cite{girgis2021renyib}.
Then, the summation over $k$ is bounded using the properties of the expected moments and the Chernoff bound (see Lemma \ref{lm:chernoff}).
The full proof is available in Appendix \ref{app:proof}.
\end{proof}
\begin{remark}
Evaluating Equation \ref{eq:main} for shuffled check-in is cumbersome as it involves a summation over the total population, $n$.
We introduce approximation techniques to speed up the evaluation as in Equation \ref{eq:upper}, which are based on Lemmas \ref{lm:chernoff} and \ref{lm:chernoff2} in Appendix \ref{app:proof}. 
Similar techniques are applicable to distributed check-in too, as will be shown in the next subsection.
\end{remark}
% While Equation \ref{eq:upper} may seem complicated, it is necessary as we attempt to obtain a precise expression (instead of an order approximation).
% This is particularly critical when considering deployment in real-life private systems, as constants matter \cite{wang2019subsampled}.
% Some numerical issues related to its evaluation will be discussed in later remarks and sections.

We next provide the corresponding lower bound.
\begin{theorem}[Lower Bound]
\label{th:lower}
For any $\eps_0\geq 0$, $n\in \mathbb{N}$, $l\leq n$ such that $0\leq\gamma \leq 1$, and any integer $\lambda\geq 2$, the RDP of the shuffled check-in mechanism is lower-bounded by
\begin{equation}
\label{eq:lower}
    \eps(\lambda)\geq\frac{1}{\lambda-1}\log\left(
1+ (1-e^{-\Delta^2n\gamma/(2+\Delta)})\binom{\lambda}{2}\gamma^2\frac{\left(e^{\epsilon_0}-1\right)^2}{(1+\Delta)n\gamma e^{\epsilon_0}}
\right),
\end{equation}
where $0 \leq \Delta \leq 1$ is arbitrary.
\end{theorem}
% \noindent \textit{Proof sketch.}
\begin{proof}[Proof sketch.]
The lower bound is calculated assuming that the underlying $\eps_0$-LDP discrete mechanism is a binary randomized response.
Again, we first obtain the expression of the subsampled without replacement (with $k$ data instances), shuffle binary randomized response.
Using the properties of the expression as well as the Chernoff bound (see Lemma \ref{lm:chernoff}), we place a lower bound on the RDP.
For the full proof, see Appendix \ref{app:proof}.
\end{proof}
% Under the setting given in the previous subsection, we derive the RDP of the shuffled check-in mechanism, which is summarized by the following theorem.




% Theorem \ref{th:main} formalizes the RDP of the shuffled check-in mechanism.
% Based on the theorem, in this section, we characterize the RDP by first presenting upper and lower RDP bounds of shuffled check-in with discrete $\eps_0$-LDP randomizer, which can be expressed in a clean and straightforward way. 
% Then, we present the procedures for calculating the generic RDP bounds, which, although computationally heavy, have wider applications.


% \subsection{RDP for shuffled check-in}
% \label{subsec:gen}
\textbf{Generic $(\eps_0,\delta_0)$-LDP randomizer.}
The bounds given above apply only to shuffled check-in with discrete $\eps_0$-LDP randomizer.
Here, we extend our consideration to generic, $(\eps_0,\delta_0)$-LDP randomizer not limited to discrete $\eps_0$-LDP mechanism.
One important application of such a consideration is the FL variant of Differentially Private SGD (DP-SGD) \citep{mcmahan2017learning,abadi2016deep}, where continuous and isotropic Gaussian noises are added to the clipped gradients.

% Let us give a sketch of our approach of bounding the RDP of a generic LDP mechanism.
Given an $(\eps_0,\delta_0)$-LDP randomizer, our strategy is to first convert it to the corresponding RDP parameters using Lemma \ref{lm:dprdp}.
The RDP parameters are then plugged into Equation \ref{eq:main} to calculate the resulting $\eps(\lambda)$.
Note that the subsampling and shuffling mechanisms' approximate DP properties are relatively well studied.
By converting them into RDP and utilizing Theorem \ref{th:main}, one can calculate the RDP of shuffled check-in in a rather straightforward way.
Note also that Equation \ref{eq:dprdp} of Lemma \ref{lm:dprdp} involves a optimization problem that cannot be written in a closed form.
Our procedure is henceforth mainly numerical (in contrast to the analytical bounds for $\eps_0$-LDP randomizer). 
We propose two approaches of tackling the problem, but showing only one in the following due to space constraints (another approach can be found in Appendix \ref{app:add}).

\noindent\textbf{Subsampled shuffling conversion.}
Our approach converts the subsampled shuffle mechanism's DP to RDP using the following procedure:
\begin{enumerate}
    \item Evaluate subsampled shuffle DP.
    \item Convert subsampled shuffle DP to subsampled shuffle RDP.
    \item Substitute it into Equation \ref{eq:main} to evaluate the composition of RDP.
\end{enumerate}
The approximate DP of subsampled shuffling can be calculated using the result of \cite{feldman2022hiding} for shuffling and Theorem 9 of \cite{balle2018privacy} for subsampling, with both having $O(1)$ time complexity. \footnote{\label{fn:shuff}
The result of privacy amplification by shuffling by \cite{feldman2022hiding} is valid only when $\eps_0 \leq \log\left(n/16\log(2/\delta)\right)$. For parameters violating this condition, we assume that no amplification occurs, i.e., $\eps=\eps_0$. 
This is well corroborated by the numerical experiments performed in \cite{feldman2022hiding}.}
The second step is a calculation of $O(\lambda)$ in terms of time complexity \citep{wang2019subsampled}, while the third step involves evaluating the summation with respect to $n$ as in Equation \ref{eq:main}, which is of $O(n)$.
Hence, in terms of time complexity with respect to $\lambda$, the overall approach takes $O(n \lambda)$. \footnote{Here, we do not include the time complexity of optimizing Equation \ref{eq:dprdp} for convenience as it is irrelevant to the subsequent discussions.
We note however that Equation \ref{eq:dprdp} is convex optimization problem which can be solved efficiently.}
% Table \ref{tab:comp} in Appendix \ref{app:add} summarizes the two approaches mentioned above.
% Although the subsampling shufffling conversion approach has lower time complexity, we expect the RDP bound to be looser than the shuffling conversion approach as the conversion to RDP occurs one step later.

\subsection{RDP for distributed check-in}
Distributed DP is perhaps the most studied method for realizing DP within the distributed setting.
While various approaches exist \citep{agarwal2018cpsgd,kairouz2021distributed,agarwal2021skellam,DBLP:journals/pvldb/BaoZXYOTA22}, most of them employ the Gaussian mechanism as the baseline. 
We henceforth analyze the use of Gaussian mechanism as the underlying randomization mechanism of the distributed check-in protocol for the ease of comparison (other mechanisms may be analyzed analogously).
Under distributed DP, we emphasize that only the aggregated values are exposed to the adversary. 

Formally, we consider each client randomizing her data instance $x_i$ of dimension $d$ with isotropic Gaussian noise of variance $\sigma^2$: $\tilde{x}_i=x_i+\mathcal{N}(0,\sigma^2I_d)$.
Here, w.l.o.g., the global sensitivity of $x_i$ is assumed to be 1 (i.e., the clipping size $C$ is set to 1).
The distributed check-in mechanism can be written as
\begin{equation}
\label{eq:cci}
    \calM(D) := \text{agg}(\{\calA(x_i)| \sigma_i=1, i \in [n]\}), \quad \sigma_i \sim \text{Bern}(\gamma).
\end{equation}
Next, we present the distributed check-in Gaussian RDP defined under replacement DP.
% This requires no further assumption on the distributed check-in protocol.
% There are two scenarios depending on whether the adversary is aware of the number of check-in in each round.

\begin{theorem}[Distributed check-in Gaussian RDP (replacement DP)]
\label{th:ssg}
Consider the mechanism in Equation \ref{eq:cci} where agg is a mean operation on collected values.
% Assume that the adversary knows the number of user checking in in each round.
Then, the RDP is
\begin{align}
    \label{eq:ssg}
\epsilon(\lambda) \leq \frac{1}{\lambda-1} \log \left(\sum_{k=1}^{n} \binom{n}{k} \gamma^{k} (1-\gamma)^{n-k} e^{(\lambda-1)\epsilon^{\rm SG}_{\gamma,k}}\right)
\end{align}
where $\epsilon^{\rm SG}$ is
\begin{align*}
    \eps^{\rm SG}_{\gamma,m}(\lambda) \leq \frac{1}{\lambda -1}
\log\left(1 + \gamma^2 \binom{\lambda}{2} \min\left\{4(e^{4/(m\sigma^2)}-1), 2 e^{4/(m\sigma^2)}\right\}
+\sum_{j=3}^{\lambda}2\gamma^j \binom{\lambda}{j} e^{2j(j-1)/(m\sigma^2)}
\right)
\end{align*}

The expression may be further approximated by
\begin{align}
\label{eq:ssg_approx}
    \epsilon(\lambda) \leq \frac{1}{\lambda-1} \log \left( e^{(\lambda-1)\epsilon^{\rm SG}_{\gamma,1}-\Delta^2n\gamma/2} +
e^{(\lambda-1)\epsilon^{\rm SG}_{\gamma,(1-\Delta)n\gamma+1}} \right)
\end{align}
with $\Delta \in [0,1]$.
\end{theorem}
\begin{proof}
At the server side, assume $k$ instances are received at certain round.
The server aggregates the data and outputs $\frac{1}{k}(\sum_{i=1}^k x_i + \mathcal{N}(0,k\sigma^2)) =\frac{1}{k}\sum_{i=1}^k x_i + \mathcal{N}(0,\sigma^2/k) $.
This mechanism has global sensitivity $2/k$ under replacement DP.
Hence, we can consider w.l.o.g. the following two base mechanisms with neighboring databases
$$
\mathcal{M}_b \sim \mathcal{N}(0, \sigma^2/k),\;\;\mathcal{M'}_b \sim \mathcal{N} (2/k, \sigma^2/k).
$$
The RDP of the base mechanism is therefore $\eps = \frac{2\lambda}{k\sigma^2}$ \citep{mironov2017renyi}.
Applying Lemma \ref{th:main} and the subsampling lemma of \cite{wang2019subsampled} leads to Equation \ref{eq:ssg}.
To obtain Equation \ref{eq:ssg_approx}, one uses monotonicity of the expression and Lemma \ref{lm:chernoff} in Appendix \ref{app:proof}.
\end{proof}
\begin{remark}
Theorem \ref{th:ssg} is derived under replacement DP.
Generally speaking, removal DP (where the adjacent database has one data instance added/removed) provides tighter bound.
To derive distributed check-in under removal DP however requires an additional trust assumption: the number of check-ins must be hidden from the adversary (otherwise, the adversary could distinguish between the neighboring databases by simply counting the number of check-ins). 
We provide the result for removal DP in Appendix \ref{app:add}.
\end{remark}




% Step 3 involves evaluating the summation with respect to $n$ as in Equation \ref{eq:main}, which is of $O(n)$.
% One also needs to convert the RDP notion back to approximate DP using Lemma \ref{lm:rdpdp}, which is an $O(\lambda)$ operation.
% Overall, the shuffling conversion approach is of time complexity $O(n\lambda^2)$. \footnote{Here, we do not include the time complexity of optimizing Equation \ref{eq:dprdp} for convenience as it is irrelevant to the subsequent discussions.
% We note however that Equation \ref{eq:dprdp} is convex optimization problem which can be solved efficiently.}

% \begin{table}
% \begin{center}
% \caption{Our approaches to bounding shuffled check-in mechanism with a generic $(\eps_0,\delta_0)$-LDP randomizer.
%     The conversion from DP to RDP (using Lemma \ref{lm:dprdp}) can be performed in two different steps leading to different time complexities as shown in the Table.
%     Dependence of the time complexity on other factors is suppressed.}
%     \label{tab:comp}

%     \begin{tabular}{ccccc}
%         \toprule
%         %\multirow{2}{*}{Dataset} &  \multicolumn{3}{c|}{social}& comm & web \\
        
%          &Shuffling&  Subsampling& Convert to RDP from & Time complexity \\
%                 \midrule
%       Approach 1& Use \cite{feldman2022hiding} (DP) &Use \cite{wang2019subsampled} (RDP)& \cite{feldman2022hiding}& $O(n\lambda\log \lambda)$ \\
%       Approach 2& Use \cite{feldman2022hiding} (DP)& Use \cite{balle2018privacy} (DP)& \cite{feldman2022hiding}+\cite{balle2018privacy}& $O(n\log \lambda)$ \\
%     %   Processing complexity& -& $n^2$& $O(\log(n))$ \\
%         \bottomrule
%     \end{tabular}
    
% \end{center}
% % \vspace{-0.2cm}
% \end{table}


==> main_results.tex <==
% Theorem \ref{th:main} formalizes the RDP of the shuffled check-in mechanism.
% Based on the theorem, in this section, we characterize the RDP by first presenting upper and lower RDP bounds of shuffled check-in with discrete $\eps_0$-LDP randomizer, which can be expressed in a clean and straightforward way. 
% Then, we present the procedures for calculating the generic RDP bounds, which, although computationally heavy, have wider applications.


% \subsection{RDP for shuffled check-in}
% \label{subsec:gen}
\textbf{Generic $(\eps_0,\delta_0)$-LDP randomizer.}
The bounds given above apply only to shuffled check-in with discrete $\eps_0$-LDP randomizer.
In this subsection, we extend our consideration to generic, $(\eps_0,\delta_0)$-LDP randomizer not limited to discrete $\eps_0$-LDP mechanism.
One important application of such a consideration is the FL variant of Differentially Private SGD (DP-SGD) \cite{mcmahan2017learning,abadi2016deep}, where continuous and isotropic Gaussian noises are added to the clipped gradients.

% Let us give a sketch of our approach of bounding the RDP of a generic LDP mechanism.
Given an $(\eps_0,\delta_0)$-LDP randomizer, our strategy is to first convert it to the corresponding RDP parameters using Lemma \ref{lm:dprdp}.
The RDP parameters are then plugged into Equation \ref{eq:main} to calculate the resulting $\eps(\lambda)$.
Note that the subsampling and shuffling mechanisms' approximate DP properties are relatively well studied.
By converting them into RDP and utilizing Theorem \ref{th:main}, one can calculate the RDP of shuffled check-in in a rather straightforward way.
Note also that Equation \ref{eq:dprdp} of Lemma \ref{lm:dprdp} involves a optimization problem that cannot be written in a closed form.
Our procedure is henceforth mainly numerical (in contrast to the analytical bounds given in the previous subsection). 
In the following, we propose two approaches of tackling the problem.

\noindent\textbf{Shuffling conversion (Approach 1).}
Our first approach proceeds as follows: 
\begin{enumerate}
    \item Convert shuffle DP to shuffle RDP.
    \item Use shuffle RDP to evaluate subsampled shuffle RDP
    \item Substitute it into Equation \ref{eq:main} to evaluate the composition of RDP.
\end{enumerate}
To calculate the shuffle DP with $(\eps_0,\delta_0)$-LDP randomizer, we use Theorem 3.8 given by \cite{feldman2022hiding}. \footnote{\label{fn:shuff}
The result of privacy amplification by shuffling by \cite{feldman2022hiding} is valid only when $\eps_0 \leq \log\left(n/16\log(2/\delta)\right)$. For parameters violating this condition, we assume that no amplification occurs, i.e., $\eps=\eps_0$. 
This is well corroborated by the numerical experiments performed in \cite{feldman2022hiding}.}
The subsampled RDP can be calculated using Theorem 9 of \cite{wang2019subsampled}.

Note that Step 2 is a calculation of $O(\lambda)$ in terms of time complexity \cite{wang2019subsampled}.
Step 3 involves evaluating the summation with respect to $n$ as in Equation \ref{eq:main}, which is of $O(n)$.
One also needs to convert the RDP notion back to approximate DP using Lemma \ref{lm:rdpdp}, which is an $O(\log\lambda)$ operation, as explained in Remark \ref{rm:logl}.
Overall, the shuffling conversion approach is of time complexity $O(n\lambda \log\lambda)$. \footnote{Here, we do not include the time complexity of optimizing Equation \ref{eq:dprdp} for convenience as it is irrelevant to the subsequent discussions.
We note however that Equation \ref{eq:dprdp} is convex optimization problem which can be solved efficiently.}

\noindent\textbf{Subsampled shuffling conversion (Approach 2).}
Our second approach converts the subsampled shuffle mechanism's DP to RDP:
\begin{enumerate}
    \item Evaluate subsampled shuffle DP.
    \item Convert subsampled shuffle DP to subsampled shuffle RDP.
    \item Substitute it into Equation \ref{eq:main} to evaluate the composition of RDP.
\end{enumerate}
The approximate DP of subsampled shuffling can be calculated using the result of \cite{feldman2022hiding} for shuffling and Theorem 9 of \cite{balle2018privacy} for subsampling, with both having $O(1)$ time complexity.
Hence, in terms of time complexity with respect to $\lambda$, the overall approach takes $O(n\log \lambda)$.
Table \ref{tab:comp} summarizes the two approaches mentioned above.
Although the subsampling shufffling conversion approach has lower time complexity, we expect the RDP bound to be looser than the shuffling conversion approach as the conversion to RDP occurs one step later.

% \begin{table}
% \begin{center}
% \caption{Our approaches to bounding shuffled check-in mechanism with a generic $(\eps_0,\delta_0)$-LDP randomizer.
%     The conversion from DP to RDP (using Lemma \ref{lm:dprdp}) can be performed in two different steps leading to different time complexities as shown in the Table.
%     Dependence of the time complexity on other factors is suppressed.}
%     \label{tab:comp}

%     \begin{tabular}{ccccc}
%         \toprule
%         %\multirow{2}{*}{Dataset} &  \multicolumn{3}{c|}{social}& comm & web \\
        
%          &Shuffling&  Subsampling& Convert to RDP from & Time complexity \\
%                 \midrule
%       Approach 1& Use \cite{feldman2022hiding} (DP) &Use \cite{wang2019subsampled} (RDP)& \cite{feldman2022hiding}& $O(n\lambda\log \lambda)$ \\
%       Approach 2& Use \cite{feldman2022hiding} (DP)& Use \cite{balle2018privacy} (DP)& \cite{feldman2022hiding}+\cite{balle2018privacy}& $O(n\log \lambda)$ \\
%     %   Processing complexity& -& $n^2$& $O(\log(n))$ \\
%         \bottomrule
%     \end{tabular}
    
% \end{center}
% % \vspace{-0.2cm}
% \end{table}
